ScissorBot: Learning Generalizable Scissor Skill for Paper Cutting via Simulation, Imitation, and Sim2Real

This paper tackles the challenging robotic task of generalizable paper cutting using scissors. In this task, scissors attached to a robot arm are driven to accurately cut curves drawn on the paper, which is hung with the top edge fixed. Due to the frequent paper-scissor contact and consequent fracture, the paper features continual deformation and changing topology, which is diffult for accurate modeling. To ensure effective execution, we customize an action primitive sequence for imitation learning to constrain its action space, thus alleviating potential compounding errors. Finally, by integrating sim-to-real techniques to bridge the gap between simulation and reality, our policy can be effectively deployed on the real robot. Experimental results demonstrate that our method surpasses all baselines in both simulation and real-world benchmarks and achieves performance comparable to human operation with a single hand under the same conditions.

==> figures/curve/curve.tex <==
\begin{figure}[ht]
    \centering
    % \vspace{-6mm}
    \includegraphics[width=0.7\linewidth]{figures/curve/curve.pdf}
    
    \vspace{-3mm}
    \caption{Example curves for Easy, Middle and Hard tracks. For Hard track in the real world, the whole pattern is cropped on an origami sheet.}
    \vspace{-2mm}
	\label{fig:curve}
\end{figure}

==> figures/ghost/ghost.tex <==
\begin{figure}[ht]
    \centering
    % \vspace{-6mm}
    \includegraphics[width=0.8\linewidth]{figures/ghost/ghost.jpg}
    
    \vspace{-3mm}
    \caption{\textbf{Visualization of Visual Artifact Mimicing} (a) Perfect point cloud in simulation with scissors blade highlighted (\textbf{\textcolor[RGB]{13,163,68}{green points}}) (b) Point cloud with our proposed visual alignment. (c) Point cloud captured in the real world with ghost noise.}
    \vspace{-2mm}
	\label{fig:ghost}
\end{figure}

==> figures/setup/setup.tex <==
\begin{figure}[ht]
    \centering
    % \vspace{-6mm}
    \includegraphics[width=0.8\linewidth]{figures/setup/real_setup.pdf}
    
    \vspace{-3mm}
    \caption{The real-world experiment setup.}
    \vspace{-2mm}
	\label{fig:setup}
\end{figure}

==> figures/setup/setup_wrap.tex <==
\begin{wrapfigure}{r}{0.4\linewidth}%靠文字内容的右侧
\centering
\vspace{-2cm}
\includegraphics[width = \linewidth]{figures/setup/real_setup.pdf}
    \vspace{-5mm}
    \caption{Hardware System.}
    \vspace{-1.5cm}
	\label{fig:setup}
\end{wrapfigure}


==> figures/teaser/teaser.tex <==
\begin{figure*}[h]
    \centering
    % \vspace{-6mm}
    \includegraphics[width=0.98\linewidth]{figures/teaser/teaser.pdf}
    
    \vspace{-3mm}
    \caption{}
    \vspace{-2mm}
	\label{fig:teaser}
\end{figure*}

==> figures/test/test.tex <==
\begin{figure*}[t]
    \centering
    \begin{tabular}{cccc}
    \includegraphics[width=0.2\linewidth]{figures/result_test.png}
    &\includegraphics[width=0.2\linewidth]{figures/result_test_notable.png}
    &\includegraphics[width=0.2\linewidth]{figures/result_test_opac.png} &\includegraphics[width=0.2\linewidth]{figures/result_test_l200.png}\\
    \end{tabular}
    \caption{just a test case of rendering}
\end{figure*}

==> tables/exp_sim_learning.tex <==
\begin{table}[htbp]
    \scriptsize
    \centering
    \begin{tabular}{l|cccc}
    \toprule
        Method  & \makecell[c]{Chamfer\\(mm)} & \makecell[c]{Recall@1.5} & \makecell[c]{Recall@5.0} \\ \midrule
        Direct Pose Regression  & $11.2^*$ & $9.0^*$ & $24.4^*$ \\ 
        \makecell[l]{Direct Pose Regression + \\ Action Chunking\cite{zhao2023learning}}  & $11.4^*$ & $8.9^*$  & $25.1^*$\\ 
        Ours  & 1.1 & 85.1 & 98.6 \\ 
        Ours  + Action Chunking\cite{zhao2023learning} & 1.2 & 84.2 & 98.5 \\ \bottomrule
    \end{tabular}
    \caption{Comparison with learning-based baselines in simulation. 
    For \textit{Direct pose regression} and its variance, we only calculate its chamber distance with the first one-third of the target curve (*). }
    \label{tab:sim_learning}
    \vspace{-2mm}
\end{table}

==> tex/02_problem.tex <==
% In this work, we study a 3D paper cutting task, where the goal is to cut a simple smooth curve or a simple pattern precisely using a scissor. 

% \subsection{Task Configurations}
% When humans cut Paper Cuttings, they tend to hold the paper with one hand to maintain stability, and operate the scissors with the other hand. 
The objective of the task is to cut a given curve or a pattern consisting of several curves on paper. To maintain the stability, the upper edge of the paper is fixed while the lower edge is set free. To achieve cutting in practice, we extended the gripper with two scissors blades. The target curve or pattern is painted in red on white paper. So the mask can be obtained through a simple segmentation based on RGB values. We use the letter-size printer paper (216mm×279mm)
with $75g/mm^2$ as material.
% Inspired by the cutting paper behavior in human beings, we aim to design a system to conduct scissor cutting while simultaneously maintaining the stabilization of the paper. 
% However, it is non-trival to design a dexterous policy to control two robot arm for one holding the scissor and the other dynamically changing grasping position and rotating the paper accordingly.
% To balance the versatility and complexity, we design a simple hardware system as shown in Fig. We use a clip to fix the upper edge of the paper, causing it to naturally sag under gravity which simulate the listing by a left hand. We attach a scissor to the Jodell robotic gripper and install it on a Realman robotic arm. We use a Kinect dk camera to capture the RGB-D images for perception. 



% \subsection{Notations}
% In the subsequent parts of this paper, we denote the intersection point in the world frame of two scissor blades as $\mathbf{P}_{\times}$. It is assumed that in both the simulator and the real world, given the angle of scissors' opening, the position of point $\mathbf{P}_{\times}$ relative to the scissors is known. During the opening and closing process of the scissors, we assume that point $\mathbf{P}_{\times}$ moves along a straight line and denote the normalized forward direction as $\mathbf{V}_{\times}$.


==> tex/intro_old.tex <==
% Paper cutting holds significant importance across various domains. 
% In the realm of kirigami, the traditional Japanese art of paper cutting and folding, intricate designs are meticulously crafted to create stunning three-dimensional structures. 
% In human society, paper cutting plays a ubiquitous role, from decorative crafts, document organization to education applications supporting creative expression in children and adults alike. Moreover, by harnessing the principles of kirigami, the traditional art of paper cutting and folding, researchers and engineers have developed novel techniques for fabricating complex structures.
% However, unlike specially designed tools for paper cutting, e.g. desktop cutting plotter, empowering robots with paper-cutting skills in 3D space is an unexplored realm, which unlocks the potential for complex and customizable designs, and advances various fields such as art, manufacturing, and education.

% Paper cutting plays a significant role in human society, serving various purposes from decorative crafts, document organization to educational applications. Moreover, by harnessing the principles of kirigami, the traditional art of paper cutting and folding, researchers and engineers have developed innovative techniques for fabricating complex structures 
Paper cutting holds great significance in human society, with applications ranging from decorative arts and document organization to educational tools. This traditional craft not only enriches cultural expression but also inspires innovative techniques in fields like engineering, where the principles of kirigami are used to create intricate and functional structures \cite{sun2015self}.
\todo{Commonly, people would use scissors to cut paper for the above purpose} \todo{What is the task: Human can easily cut any line on a piece of paper.} However, empowering robots with paper-cutting skills using scissors remains an unexplored realm. \todo{Especially learning base method.} Unlike using specially designed tools like desktop cutting plotters, this robotic skill in using scissors holds the potential for producing complex and customizable designs, thus benefiting diverse fields such as art, manufacturing, and education.

% The art of paper cutting holds significant importance in various domains, from origami-inspired tool design to the intricate maneuvers of kirigami robots. However, when we extend this practice to three-dimensional realms, new challenges emerge, necessitating the development of specialized robotic capabilities.

% For 3D paper cutting, challenges arise due to the deformable nature of the paper. First, the fracture of the paper introduces complexities that are difficult to model accurately, giving rise to intricate patterns of vision and physics properties. Additionally, the interaction between scissors and paper introduces occasional occlusion for visual perception and highly non-linear dynamics for physics. Even millimetric movements may lead to either drastic bending (Fig.\ref{fig:teaser}) in the paper or a visually distant curve with the target.

\todo{The correlation between 'application' and 'challenge'. }
The task of paper cutting with scissors is challenging which features highly nonlinear dynamics due to the deformable nature and fracture of the paper. 
Even millimetric scissor movements may lead to either drastic bending (Fig.\ref{fig:teaser}) in the paper or a visually distant curve with the target. 
% Second, the fracture phenomenon introduces intricate visual patterns and physical property.
In addition, the area on the paper around the fracture is more fragile and easily torn by the action of scissors, raising high demands for fine operation.
The scissors also occasionally occlude the target curve, making the decision-making problem ill-posed during these steps.
% These challenges poses significant obstacles to achieving fault-tolerant control strategies but demands high levels of accurate operation.


Considering the difficulty of designing rules for cutting in such complex scenarios, learning-based methods have the potential to achieve generalization, which benefits from data-driven. However, learning such precise cutting skills directly on a real-world robot system is challenging, time-consuming and potentially dangerous. Moreover, existing simulators for thin-thell objects\cite{wang2024thin, lin2021softgym, chen2022daxbench} in the literature don't support interactive   fracture coupling with rigid bodies.
%Moreover, existing simulators in the literature are limited in simulating thin-thell objects supporting detailed interaction with rigid bodies, including contact and consequent fracture.

Meanwhile, data coming from simulation have a significant sim2real gap including both visual and physical perspectives. The physics gap sometimes leads to the drifting of cutting trajectory.
The visual gap, mainly ghost noise from depth sensor, jitters the observation of interaction between scissors and paper, leading to incorrect policy decisions. 

To address the above challenges, we introduce ScissorBot, the first learning-based
strategy for paper cutting with scissors via a combination of simulation, imitation learning and sim2real. 
To mitigate the data scarcity issue, we developed the first paper-cutting simulator supporting interactive fracture coupling with scissors, PaperCutting-Sim, which enables us to conduct heuristic-based demonstration generation with an oracle policy.

In facing the highly non-linear dynamics, reinforcement learning without carefully designed dense reward struggles to learn a long-horizon policy effectively. 
Imitation learning with direct pose regression suffers a lot from distribution shift, as action with small errors will cause many different states from those in the training data.
To this end, we proposed several primitives to constrain the action space of imitation learning and fix their execution order, achieving robust execution. We also use spatial-temporal encoding \todo{multi frame point cloud} to predict action under occlusion. Temporal inputs complete the occluded information and contain deformable dynamic cues, which is beneficial to the prediction of accurate actions.

% The well-designed primitives constrain the DoF of scissor motion, which contributes to alleviate potential compounding errors. 
% Moreover, we leverage spatial-temporal observation encoding to empower accurate prediction under occlusion.

% To address the above challenges, we introduce primitive learning rather than direct pose regression for imitation learning. The well-designed primitives constrain the DoF of scissor motion, which contributes to alleviate potential compounding errors. 
% Moreover, we leverage spatial-temporal observation encoding to empower accurate prediction under occlusion.


% However, learning such precise cutting skills directly on a real-world robot system is challenging, time-consuming and potentially dangerous. Moreover, existing simulators \cite{wang2024thin, lin2021softgym, chen2022daxbench} in the literature are limited in simulating thin-thell objects supporting detailed interaction with scissors including contact and consequent fracture. Therefore, we develop the first paper-cutting simulator, PaperCutting-Sim, allowing us to design an oracle policy to generate expert demonstration for distillation.

% Crucially, we observe that directly deploying the policy into the real-world system suffers a lot from sim2real gap including both physical and visual perspectives. The physics gap \todo{often} leads to the drifting of cutting trajectory. To this end, we propose Deviation Correction to adaptively correct compounding errors and enhance the robustness. Meanwhile, the visual gap, mainly ghost noise from depth sensor, jitters the observation of interaction between scissors and paper, leading to incorrect policy predictions. Thus, we design a simple yet effective method to mimic this phenomenon, achieving visual alignment between simulation and reality. 

To deal with physical and visual gaps between simulation and reality, we propose data augmentation on deviation correction and ghost noise handling, respectively. 
The former method can adaptively correct compounding errors via adding out-of-distribution data which pairs deviation states with corresponding correction action. The latter aims to mimic ghost noise in the simulation to achieve visual alignment with reality.
% We also use deviation correction to adaptively correct compounding errors through a data augmentation method. we design a simple yet effective method to mimic ghost noise achieving visual alignment between simulation and reality.
% We also tackle discrepancies arising from differences in simulation and real-world depth perception through Visual Alignment. 
Through comprehensive validation, our policy can cut diverse curves and patterns that are harder than training distribution in both simulation and real world, which achieve a near-human single-hand performance for our test cases.
% In summary, the primary contribution of this paper is the first robotic system demonstrating the capability of 3D paper cutting. To build this system, we make the following technical advancements:

% \begin{enumerate}
%     \item The formulation of the 3D paper cutting task and a simulator that could perform realistic interaction modeling between paper and scissors for collecting demonstrations.

%     \item A learning-based cutting method with an stage-wise constrained action space and 4D temporal perception.

%     \item Divation correction and Visual Alignmnet for Sim2real transfer and the deployment of our method on a real-world robotic system.
% \end{enumerate}
% In summary, our proposed Sim2Real approach offers a holistic solution to the challenges inherent in robotic 3D paper cutting. Through a fusion of simulation, imitation learning, and robust transfer to real-world environments, we pave the way for practical applications of this intricate manipulation task, underscoring its potential to advance the field of robotic manipulation for deformable objects.

In summary, the key contribution of this paper is ScissorBot, the first learning-based robotic system demonstrating scissor skills for paper cutting. To build this system,
we make the following technical advancements: i) The first paper-cutting simulator, PaperCutting-Sim, which simulates contacts and the consequent fracture of paper and scissors, ii) an imitation learning method combined with spatial-temporal observation encoding and primitive learning for robust and accurate cutting.
iii) two sim2real techniques, namely deviation correction and ghost noise handling, for the successful deployment of our policy on a real-world robotic system.

% Videos of experiments, the code for the simulator and the cutting system, as well as the CAD models for the benchmark
% objects are available at

==> tex/simulation_old.tex <==
Due to the necessity of modifying the topology of the paper based on the relative positions of scissors and paper, there is currently no physical simulator well-suited for our task. Therefore, we have built our own simulator. 

Our paper-cutting simulator mainly uses Taichi programming language \cite{hu2019taichi}. Taichi is proficient in leveraging GPU for large-scale parallel simulations and offers convenient Python APIs. The elastic force simulation within the paper is based on the finite element method (FEM) and implicit time integration \cite{baraff2023large}. We also handle collisions between scissors and paper in our simulation. As for paper fracture handling, unlike the previous approaches \cite{pfaff2014adaptive} that directly consider the forces within the paper to compute where to break, we employed a purely geometry-based approach to modify the topology of the paper mesh to avoid considering the complex fracture mechanics of paper. 

\subsubsection{Paper Simulation}

Paper can be approximated as a two-dimensional manifold, and we model it using a triangular mesh. Stretching elastic potential energy is defined on each triangle, modeled using \textit{co-rotational linear elasticity}. Bending elastic potential energy is defined on the dihedral angle formed by two adjacent triangles, with energy proportional to the square of the dihedral angle \cite{pfaff2014adaptive}. Due to the emergence of numerous small triangles in the paper mesh during the paper cutting process, explicit time integration becomes highly unstable. Therefore, we employ implicit time integration \cite{baraff2023large} to ensure the robustness of the simulation. 

% \subsubsection{Collision}
% Considering that self-collisions of paper rarely occur during the cutting process with scissors, our simulator only takes into account collisions between scissors and paper. The collision model for scissors is represented as a signed distance function (SDF) and the collision energy between paper and scissors is modeled as a cubic function. 

For scissors, a kind of rigid body, we represent them as time-varying signed distance fields (SDFs), converted from imported external meshes. We model the contact between
thin-thell and rigid materials by computing surface normals of the
SDFs and applying Coulomb friction. Material separation occurring during the cutting process is handled by our designed Fracture Handling.
\subsubsection{Fracture Handling}

The procedure for handling paper cutting process is summarized in algorithm \ref{alg:cutsim}. Paper fracture will be handled at each time step.

\begin{algorithm}[h]
\caption{Cutting Simulation}
\label{alg:cutsim}
\begin{algorithmic}

\State \textbf{Input:} scissors state $S$, paper mesh $M$
\State \textbf{Output:} new scissors state $S'$, new paper mesh $M'$

\If {\Call{isCuttingState}{$S$}}
    \State $M_v, v$ $\gets$ \Call{insertNewVert}{$M,S$}
    \State $M'$ $\gets$ \Call{splitEdge}{$M_v, v$}
    \State $S'$ $\gets$ $S$
\Else
    \State $S'$ $\gets$ \Call{constrainScissors}{$S$}
    \State $M'$ $\gets$ $M$
\EndIf
\State
\Function{insertNewVert}{$M,S$}
    \State Hyperparameters $\alpha,\beta$
    \State calculate $\mathbf{P}_\times, \mathbf{V}_\times$ using $S$
    \State Init $v$ $\gets$ emptySet(), $E$ $\gets$ $Edge\{\mathbf{P}_\times, \mathbf{P}_\times - \alpha\mathbf{V}_\times\}$
    \For{$e$ in $M$.edges}
        \If {$\textit{dist}(e, E)<\beta$}
            \State calculate nearest pair $(x,X)$: $x\in e,X\in E$
            \State $v$.\Call{add}{$M$.\Call{snapInsert}{$x$}}
        \EndIf
    \EndFor
    
    \For{$f$ in $M$.faces}
        \If {$\textit{dist}(f, \mathbf{P}_\times)<\beta$}
            \State calculate nearest point $x$: $x\in f$
            \State $v$.\Call{add}{$M$.\Call{snapInsert}{$x$}}
        \EndIf
    \EndFor
    \State \Return $M, v$
\EndFunction
\State
\Function{splitEdge}{$M, v$}
    \For{$i$ in $v$}
        \For{$j$ in $v$}
            \If {$M$.\Call{existInternalEdge}{$i,j$}}
                \State $M$.\Call{split}{$i,j$}
            \EndIf
        \EndFor
    \EndFor
\EndFunction

\end{algorithmic}
\end{algorithm}

Firstly, we determine whether the scissors are in a paper-cutting state. If the closing angular velocity of the scissors is positive, then \textit{isCuttingState} returns True; otherwise, it returns False. When the scissors are in a paper-cutting state, based on the pose of the scissors and the mesh of the paper, we add new vertices and split the mesh along some edges. When the scissors are not in a paper-cutting state, we impose constraints on the actions of the scissors to prevent the scissors from making unreasonable actions such as directly pushing inward.

% We add these constraints because our control of the scissors is based on position, without any feedback from the paper to the scissors. If the scissors were to perform unreasonable actions (such as directly inserting into the paper), it would pose serious challenges to the simulation of the paper. To prevent the scissors from making such actions, we impose specific constraints on the actions of the scissors.

%\textbf{Determining cutting state}

\textbf{Inserting new vertices:} Let $E$ be the segment where the blade is located and $M$ be the mesh of the paper. Refer to the function \textit{insertNewVert}, the core idea is to compute the intersection between $E$ and $M$. The two endpoints of $E$ is located are $\mathbf{P}_\times$ and $\mathbf{P}_\times-\alpha\mathbf{V}_\times$, where $\alpha$ is a hyper-parameter and represents the length of the segment. Then performing edge-edge detection and vertex-face detection will yield all intersection points on $M$.

\textbf{Robustly inserting:} Assuming we want to insert a new vertex at position $x$ on the mesh, let's first consider the naive approach: inserting the vertex directly. This approach results in new triangles with unrestricted sizes, leading to many small triangles. Moreover, as the time step decreases, the movement of the scissors in each time step also decreases, resulting in even smaller triangles. These small triangles can easily destabilize force-based physical simulations. To ensure robustness when adding new vertices, we propose the \textit{snapInsert} function. If $x$ is too close to an existing vertex on the grid (smaller then a threshold $\delta$), we directly snap (attach) the new vertex to the existing one and return the existing vertex.

\textbf{Remeshing.}

\textbf{Splitting existing edges:} The function \textit{insertNewVert} will return a set of vertices that need to be split, which may consist of both existing vertices and newly inserted vertices. Subsequently, iterating through pairs of vertices in this set. If the two vertices in a pair are connected by an internal edge of the mesh (i.e., both sides of the edge have triangular faces), then the mesh is split along this edge.

\textbf{Constraints on the scissors:} The function \textit{constrainScissors} only allows the scissors to rotate, move along the opposite direction of $\mathbf{V}_\times$, or perform opening and closing actions. This prevents the scissors from attempting to penetrate the paper by rudely pushing inward.
